STALL+: Boosting LLM-based Repository-level Code Completion with Static Analysis

Repository-level code completion is challenging as it involves complicated contexts from multiple files in the repository. To date, researchers have proposed two technical categories to enhance LLM-based repository-level code completion, i.e., retrieval-augmented generation (RAG) and static analysis integration. This work performs the first study on the static analysis integration in LLM-based repository-level code completion by investigating both the effectiveness and efficiency of static analysis integration strategies across different phases of code completion. We first implement a framework STALL+, which supports an extendable and customizable integration of multiple static analysis strategies into the complete pipeline of LLM-based repository-level code completion; and based on STALL+, we perform extensive experiments by including different code LLMs on the latest repository-level code completion benchmark CrossCodeEval. Our findings show that integrating file-level dependencies in prompting phase performs the best while the integration in post-processing phase performs the worse. Additionally, we observe different improvements from static analysis between dynamic languages and static languages, i.e., the best combination is prompting-phase with decoding-phase integration for Java while the best combination is prompting-phase with post-processing-phase integration for Python given the limitations of statically analyzing dynamic languages. Additionally, we find the complementarity between RAG and static analysis integration as well as their cost-effectiveness after combination.

==> sections/RQ/rq4.tex <==
\subsection{RQ4: Do \analysisaugmented{} methods vary in effectiveness between dynamic and static type languages?}
\textbf{Motivation.}
Programming languages fall into two main categories: statically and dynamically typed. 
Dynamically typed languages, \eg{} Python and JavaScript, defer variable typing at runtime, while statically typed languages, such as C++ and Java, determine variable types at compile time, facilitating a more straightforward process for conducting static analysis. 
Given the inherent discrepancies in the accuracy of static analysis, in this RQ, we aim to investigate the differences in using \analysisaugmented{} methods between statically typed languages and dynamically typed languages.

\textbf{Approach.}
We select two popular programming languages, Python and Java, as the representative of dynamically typed languages and statically typed languages, respectively.
Since CrossCodeEval benchmark comprises datasets for Python both Java, we directly conduct experiments of different methods on these two subsets and compare the results.

\textbf{Results.}
Experimental results on different models are shown in Table ~\ref{tab:deepseek-coder}, ~\ref{tab:starcoder} and ~\ref{tab:codellama}. 



\smalltitle{Comprison of \si{} and \sls{}.}
Firstly, while \si{} and \sls{} can improve the accuracy of repository-level line completion on both Python and Java datasets, a slightly higher absolute improvement can be observed in Python. Considering that the prediction accuracy of \infile{} on Python is much lower, we further calculate the relative improvement and find that \si{} can achieve more than 200\% relative improvement on Python, while the relative improvement is less than 100\% on Java, further demonstrating the efficiency of \analysisaugmented{} methods on Python.

\smalltitle{Comprison of \sd{} and \spo{}.}
As discussed in RQ2, on the Python dataset, the \sd{} method often fails to further improve accuracy when combined with other static analysis methods. Conversely, on Java data, the \sd{} method demonstrates a noticeable enhancement, particularly when combined with \si{}, which is more complementary.

For the \sd{} method, if static analysis cannot obtain the correct API, the result is unlikely to be accurate. 
Therefore, compared to other methods, it relies more heavily on the accuracy of static analysis. 
However, Dynamically typed languages do not confirm types at compile time and have more flexible syntax, making static analysis more challenging. 
This increases the probability of errors and misjudgments in completion. 
Consequently, relying on static analysis for results leads to significant biases in dynamically typed languages. 
However, in statically typed languages like Java, \sd{} method can still lead to distinctly positive gains.

For similar reasons, \spo{} also shows a higher improvement on the Java dataset compared to the Python dataset.

\smalltitle{Comprison in cost.} \todo{move to RQ5?}
The \spo{} method, as well as methods incorporating \spo{} such as \sip{} and \slsp{}, all demonstrate faster execution speed on Java. Conversely, the \sd{} method exhibits faster execution on Python.\todo{why?}

\finding{Overall, Various \analysisaugmented{} methods can effectively improve the accuracy of both dynamically and statically typed languages. \sd{} and \spo{} both demonstrate better enhancement on Java compared to Python. Furthermore, conducting static analysis on statically typed languages costs relatively lower inference time.}

==> tables/codellama.tex <==
\begin{table*}[htp]
\centering
\caption{Results for \codellama{} on line-level code completion.}
\label{tab:codellama}
\begin{adjustbox}{width=2.1\columnwidth}
\begin{tabular}{c|c|cc|cc|c|cc|cc|c}
\hline
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                                                                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                  & \multicolumn{5}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Python}}                                                                                                                                                                                                                                                           & \multicolumn{5}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Java}}                                                                                                                                                                                                                 \\ \cline{3-12} 
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                                                                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                  & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Code Match}}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Identifier Match}}                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Time}}       & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Code Match}}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Identifier Match}}                                              & \textbf{Time}       \\ \cline{3-12} 
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{F2F2F2}\textbf{\begin{tabular}[c]{@{}c@{}}Augmented\\ Type\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{F2F2F2}\textbf{Method}}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Line EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Line ES}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{F1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{cost(s/it)}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Line EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Line ES}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{F1}} & \textbf{cost(s/it)} \\ \hline
\textbf{None} & \textbf{\infile{}} & 7.20 & 60.69 & 13.94 & 45.62 & 1.12 & 25.59 & 72.85 & 33.45 & 57.97 & 2.07 \\ \hline
\textbf{Retrieval} & \textbf{RG-1} & 17.52(↑10.32) & 67.71(↑7.02) & 26.22(↑12.28) & 56.41(↑10.79) & 1.95(↑0.83) & 35.90(↑10.31) & 76.91(↑4.06) & 44.58(↑11.13) & 66.15(↑8.18) & 1.99(↓0.08) \\ \hline
 & \textbf{S-I} & 23.94(↑16.74) & 69.77(↑9.08) & 33.01(↑19.07) & 61.18(↑15.56) & 1.85(↑0.73) & 41.25(↑15.66) & 78.79(↑5.94) & 50.99(↑17.54) & 71.12(↑13.15) & 1.90(↓0.17) \\
 & \textbf{S-LS} & 21.46(↑14.26) & 67.34(↑6.65) & 30.33(↑16.39) & 58.11(↑12.49) & 1.53(↑0.41) & 33.35(↑7.76) & 74.95(↑2.10) & 42.46(↑9.01) & 64.82(↑6.85) & 1.39(↓0.68) \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Static\\ Analysis\end{tabular}}} & \textbf{S-P} & 8.87(↑1.67) & 60.47(↓0.22) & 14.92(↑0.98) & 45.84(↑0.22) & 7.48(↑6.36) & 27.66(↑2.07) & 72.63(↓0.22) & 35.47(↑2.02) & 58.73(↑0.76) & 4.80(↑2.73) \\ \hline
 & \textbf{S-I-P} & 25.22(↑1.28) & 69.27(↓0.50) & 33.31(↑0.30) & 60.39(↓0.79) & 9.00(↑7.15) & 43.28(↑2.03) & 79.05(↑0.26) & 52.58(↑1.59) & 71.84(↑0.72) & 6.67(↑4.77) \\
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Combined\\Static  Analysis\end{tabular}}} & \textbf{S-LS-P} & 24.09(↑2.63) & 67.76(↑0.42) & 32.03(↑1.70) & 58.75(↑0.64) & 9.40(↑7.87) & 36.14(↑2.79) & 75.45(↑0.50) & 44.82(↑2.36) & 66.11(↑1.29) & 5.22(↑3.83) \\ \hline
 & \textbf{RG-1 + S-I} & 29.55(↑5.61) & {\ul \textbf{73.86(↑4.09)}} & 40.49(↑7.48) & {\ul \textbf{67.23(↑6.05)}} & 2.72(↑0.87) & 47.61(↑6.36) & 81.30(↑2.51) & 57.45(↑6.46) & 75.58(↑4.46) & 2.71(↑0.81) \\
 & \textbf{RG-1 + S-LS} & 27.32(↑5.86) & 70.94(↑3.60) & 37.64(↑7.31) & 63.56(↑5.45) & 2.33(↑0.80) & 41.98(↑8.63) & 78.59(↑3.64) & 51.33(↑8.87) & 70.81(↑5.99) & 2.17(↑0.78) \\
 & \textbf{RG-1 + S-P} & 19.59(↑10.72) & 68.16(↑7.69) & 27.52(↑12.60) & 56.83(↑10.99) & 7.90(↑0.42) & 38.36(↑10.70) & 77.39(↑4.76) & 46.89(↑11.42) & 67.37(↑8.64) & 7.06(↑2.26) \\
 & \textbf{RG-1 + S-I-P} & {\ul \textbf{31.34(↑6.12)}} & 73.48(↑4.21) & {\ul \textbf{40.93(↑7.62)}} & 66.58(↑6.19) & 11.54(↑2.54) & {\ul \textbf{48.72(↑5.44)}} & {\ul \textbf{81.46(↑2.41)}} & {\ul \textbf{58.22(↑5.64)}} & {\ul \textbf{75.86(↑4.02)}} & 9.25(↑2.58) \\
\multirow{-5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Retrieval\\  + \\ Static\\ Analysis\end{tabular}}} & \textbf{RG-1 + S-LS-P} & 29.07(↑5.48) & 70.86(↑3.64) & 38.62(↑6.78) & 63.34(↑5.49) & 10.52(↑2.49) & 43.90(↑7.76) & 78.92(↑3.47) & 52.63(↑7.81) & 71.89(↑5.78) & 7.63(↑2.41) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/deepseek-coder.tex <==
\begin{table*}[htp]
\centering
\caption{Results for \deepseekcoder{} on line-level code completion.
While ``Retrieval'' and ``Static Analysis'' enhancements are absolute improvements relative to ``\infile{}'', the improvements in ``Static Analysis (Combined)'' are relative to its base methods: \si{}/\sls{} and ``Retrieval + Static Analysis'' improvements are relative to the \analysisaugmented{} methods it contains.
The tables of other models follow the same representation rules.}
\label{tab:deepseek-coder}
\begin{adjustbox}{width=2.1\columnwidth}
\begin{tabular}{c|c|cc|cc|c|cc|cc|c}
\hline
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                                                                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                  & \multicolumn{5}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Python}}                                                                                                                                                                                                                                                           & \multicolumn{5}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Java}}                                                                                                                                                                                                                 \\ \cline{3-12} 
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                                                                    & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}}                                  & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Code Match}}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Identifier Match}}                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Time}}       & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Code Match}}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Identifier Match}}                                              & \textbf{Time}       \\ \cline{3-12} 
\rowcolor[HTML]{F2F2F2} 
\multicolumn{1}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{F2F2F2}\textbf{\begin{tabular}[c]{@{}c@{}}Augmented\\ Type\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{-3}{*}{\cellcolor[HTML]{F2F2F2}\textbf{Method}}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Line EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Line ES}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{F1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{cost(s/it)}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Line EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Line ES}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{F1}} & \textbf{cost(s/it)} \\ \hline
\textbf{None} & \textbf{Infile} & 9.02 & 62.51 & 15.45 & 48.00 & 1.12 & 26.70 & 73.38 & 34.36 & 58.62 & 1.20 \\ \hline
\textbf{Retrieval} & \textbf{RG-1} & 20.33(↑11.31) & 69.50(↑6.99) & 29.27(↑13.82) & 59.16(↑11.16) & 1.96(↑0.84) & 38.27(↑11.57) & 78.04(↑4.66) & 47.13(↑12.77) & 67.81(↑9.19) & 1.97(↑0.77) \\ \hline
 & \textbf{S-I} & 27.80(↑18.78) & 72.64(↑10.13) & 36.75(↑21.30) & 64.94(↑16.94) & 1.70(↑0.58) & 44.24(↑17.54) & 80.33(↑6.95) & 53.25(↑18.89) & 73.19(↑14.57) & 1.88(↑0.68) \\
 & \textbf{S-LS} & 24.84(↑15.82) & 69.89(↑7.38) & 33.94(↑18.49) & 61.70(↑13.70) & 1.53(↑0.41) & 38.65(↑11.95) & 76.95(↑3.57) & 47.18(↑12.82) & 68.42(↑9.80) & 1.42(↑0.22) \\
 & \textbf{S-D} & 16.02(↑7.00) & 63.92(↑1.41) & 23.37(↑7.92) & 54.30(↑6.30) & 5.72(↑4.60) & 33.11(↑6.41) & 74.34(↑0.96) & 41.45(↑7.09) & 64.49(↑5.87) & 8.92(↑7.72) \\
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Static\\ Analysis\end{tabular}}} & \textbf{S-P} & 11.54(↑2.52) & 63.39(↑0.88) & 17.36(↑1.91) & 49.44(↑1.44) & 9.78(↑8.66) & 30.36(↑3.66) & 73.63(↑0.25) & 38.07(↑3.71) & 60.96(↑2.34) & 4.66(↑3.46) \\ \hline
 & \textbf{S-I-D} & 28.01(↑0.21) & 70.83(↓1.81) & 36.38(↓0.37) & 63.98(↓0.96) & 5.51(↑3.81) & 46.46(↑2.22) & 80.68(↑0.35) & 55.37(↑2.12) & 75.18(↑1.99) & 8.78(↑6.90) \\
 & \textbf{S-I-P} & 28.74(↑0.94) & 72.40(↓0.24) & 36.91(↑0.16) & 65.04(↑0.10) & 10.50(↑8.80) & 45.93(↑1.69) & 80.49(↑0.16) & 54.80(↑1.55) & 73.79(↑0.60) & 5.10(↑3.22) \\
 & \textbf{S-LS-D} & 24.51(↓0.33) & 68.08(↓1.81) & 32.80(↓1.14) & 60.55(↓1.15) & 5.72(↑4.19) & 39.04(↑0.39) & 76.53(↓0.42) & 47.47(↑0.29) & 68.44(↑0.02) & 8.11(↑6.69) \\
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Combined\\ Static\\ Analysis\end{tabular}}} & \textbf{S-LS-P} & 26.95(↑2.11) & 70.05(↑0.16) & 35.45(↑1.51) & 61.99(↑0.29) & 9.60(↑8.07) & 40.34(↑1.69) & 76.97(↑0.02) & 48.48(↑1.30) & 69.01(↑0.59) & 5.17(↑3.75) \\ \hline
 & \textbf{RG-1 + S-I} & 33.66(↑5.86) & 75.94(↑3.30) & 44.02(↑7.27) & 70.06(↑5.12) & 2.73(↑1.03) & 50.70(↑6.46) & 82.71(↑2.38) & 60.29(↑7.04) & 77.54(↑4.35) & 2.69(↑0.81) \\
 & \textbf{RG-1 + S-LS} & 30.61(↑5.77) & 73.67(↑3.78) & 41.18(↑7.24) & 67.38(↑5.68) & 2.36(↑0.83) & 45.16(↑6.51) & 80.23(↑3.28) & 54.65(↑7.47) & 73.77(↑5.35) & 2.15(↑0.73) \\
 & \textbf{RG-1 + S-D} & 24.02(↑8.00) & 68.45(↑4.53) & 32.89(↑9.52) & 61.25(↑6.95) & 6.00(↑0.28) & 42.80(↑9.69) & 78.71(↑4.37) & 51.56(↑10.11) & 71.48(↑6.99) & 8.82(↓0.10) \\
 & \textbf{RG-1 + S-P} & 22.93(↑11.39) & 70.29(↑6.90) & 31.06(↑13.70) & 60.08(↑10.64) & 11.48(↑1.70) & 40.92(↑10.56) & 78.15(↑4.52) & 49.35(↑11.28) & 68.98(↑8.02) & 6.98(↑2.32) \\
 & \textbf{RG-1 + S-I-D} & 32.32(↑4.31) & 73.32(↑2.49) & 41.30(↑4.92) & 67.49(↑3.51) & 6.79(↑1.28) & {\ul \textbf{52.05(↑5.59)}} & {\ul \textbf{82.96(↑2.28)}} & {\ul \textbf{61.40(↑6.03)}} & {\ul \textbf{78.81(↑3.63)}} & 9.41(↑0.63) \\
 & \textbf{RG-1 + S-I-P} & {\ul \textbf{34.67(↑5.93)}} & {\ul \textbf{76.51(↑4.11)}} & {\ul \textbf{45.00(↑8.09)}} & {\ul \textbf{70.55(↑5.51)}} & 12.75(↑2.25) & {\ul \textbf{52.05(↑6.12)}} & 82.41(↑1.92) & 60.87(↑6.07) & 77.48(↑3.69) & 8.35(↑3.25) \\
 & \textbf{RG-1 + S-LS-D} & 29.31(↑4.80) & 71.21(↑3.13) & 38.54(↑5.74) & 64.87(↑4.32) & 6.34(↑0.62) & 45.20(↑6.16) & 79.93(↑3.40) & 54.46(↑6.99) & 73.68(↑5.24) & 9.36(↑1.25) \\
\multirow{-8}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Retrieval\\  + \\ Static Analysis\end{tabular}}} & \textbf{RG-1 + S-LS-P} & 32.36(↑5.41) & 74.00(↑3.95) & 42.11(↑6.66) & 67.58(↑5.59) & 12.17(↑2.57) & 46.75(↑6.41) & 80.54(↑3.57) & 56.29(↑7.81) & 74.76(↑5.75) & 5.78(↑0.61) \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/settings.tex <==
\begin{table}[]
\centering
\caption{Settings}
\label{tab:settings}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Name  & Infile Context & Import Context & Retreival Context & Language Server Context & Decoding Intervention & Post-processing \\ \hline
I     & √              & ×              & ×                 & ×                       & ×                     & ×               \\ \hline
RG-1  & √              & ×              & √                 & ×                       & ×                     & ×               \\ \hline
S-I   & √              & √              & ×                 & ×                       & \textbf{×}            & ×               \\ \hline
S-LS  & √              & ×              & ×                 & √                       & ×                     & ×               \\ \hline
S-D   & √              & ×              & ×                 & ×                       & √                     & ×               \\ \hline
S-P   & √              & ×              & ×                 & ×                       & ×                     & √               \\ \hline
S-I-D & √              & √              & ×                 & ×                       & \textbf{√}            & ×               \\ \hline
S-I-P & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
      & √              &                &                   &                         &                       &                 \\ \hline
\end{tabular}
\end{table}

==> tables/starcoder.tex <==
\begin{table*}[htp]
\centering
\caption{Results for \starcoder{} on line-level code completion.}
\label{tab:starcoder}
\begin{adjustbox}{width=2.1\columnwidth}
\begin{tabular}{c|c|cc|cc|c|cc|cc|c}
\hline
\rowcolor[HTML]{F2F2F2} 
\cellcolor[HTML]{F2F2F2}                                                                                    & \cellcolor[HTML]{F2F2F2}                                  & \multicolumn{5}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Python}}                                                                                                                                                                                                              & \multicolumn{5}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Java}}                                                                                                                                                                                                                \\ \cline{3-12} 
\rowcolor[HTML]{F2F2F2} 
\cellcolor[HTML]{F2F2F2}                                                                                    & \cellcolor[HTML]{F2F2F2}                                  & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Code Match}}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Identifier Match}}                                              & \textbf{Time}       & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Code Match}}                                                              & \multicolumn{2}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Identifier Match}}                                              & \textbf{Time}       \\ \cline{3-12} 
\rowcolor[HTML]{F2F2F2} 
\multirow{-3}{*}{\cellcolor[HTML]{F2F2F2}\textbf{\begin{tabular}[c]{@{}c@{}}Augmented\\ Type\end{tabular}}} & \multirow{-3}{*}{\cellcolor[HTML]{F2F2F2}\textbf{Method}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Line EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Line ES}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{F1}} & \textbf{cost(s/it)} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{Line EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{Line ES}} & \multicolumn{1}{c}{\cellcolor[HTML]{F2F2F2}\textbf{EM}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F2F2F2}\textbf{F1}} & \textbf{cost(s/it)} \\ \hline
\textbf{None} & \textbf{\infile{}} & 6.38 & 60.82 & 13.17 & 45.53 & 1.04 & 23.61 & 72.22 & 32.24 & 56.95 & 1.01 \\ \hline
\textbf{Retrieval} & \textbf{RG-1} & 16.06(↑9.68) & 67.07(↑6.25) & 25.28(↑12.11) & 55.84(↑10.31) & 1.77(↑0.73) & 34.12(↑10.51) & 76.42(↑4.20) & 44.00(↑11.76) & 65.81(↑8.86) & 1.75(↑0.74) \\ \hline
 & \textbf{S-I} & 23.58(↑17.20) & 69.78(↑8.96) & 32.20(↑19.03) & 61.35(↑15.82) & 1.69(↑0.65) & 40.19(↑16.58) & 78.90(↑6.68) & 50.60(↑18.36) & 71.23(↑14.28) & 1.67(↑0.66) \\
 & \textbf{S-LS} & 20.28(↑13.90) & 66.31(↑5.49) & 28.62(↑15.45) & 56.49(↑10.96) & 1.40(↑0.36) & 34.51(↑10.90) & 75.72(↑3.50) & 44.19(↑11.95) & 66.09(↑9.14) & 2.53(↑1.52) \\
 & \textbf{S-D} & 13.09(↑6.71) & 62.21(↑1.39) & 20.73(↑7.56) & 52.13(↑6.60) & 4.33(↑3.29) & 30.89(↑7.28) & 73.75(↑1.53) & 39.90(↑7.66) & 63.37(↑6.42) & 9.61(↑8.60) \\
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Static\\ Analysis\end{tabular}}} & \textbf{S-P} & 7.73(↑1.35) & 60.32(↓0.50) & 13.70(↑0.53) & 45.78(↑0.25) & 6.24(↑5.20) & 26.12(↑2.51) & 72.46(↑0.24) & 34.89(↑2.65) & 58.20(↑1.25) & 4.23(↑3.22) \\ \hline
 & \textbf{S-I-D} & 23.98(↑0.40) & 68.20(↓1.58) & 31.42(↓0.78) & 60.40(↓0.95) & 5.87(↑4.18) & 42.89(↑2.70) & 79.24(↑0.34) & 53.25(↑2.65) & 73.56(↑2.33) & 9.70(↑8.03) \\
 & \textbf{S-I-P} & 25.09(↑1.51) & 70.10(↑0.32) & 32.94(↑0.74) & 61.92(↑0.57) & 9.03(↑7.34) & 41.73(↑1.54) & 78.89(↓0.01) & 51.76(↑1.16) & 71.20(↓0.03) & 11.33(↑9.66) \\
 & \textbf{S-LS-D} & 20.81(↑0.53) & 64.62(↓1.69) & 28.53(↓0.09) & 55.57(↓0.92) & 5.70(↑4.30) & 35.04(↑0.53) & 75.46(↓0.26) & 44.82(↑0.63) & 66.38(↑0.29) & 9.60(↑7.07) \\
\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Combined\\Static\\ Analysis\\ \end{tabular}}} & \textbf{S-LS-P} & 22.34(↑2.06) & 66.53(↑0.22) & 29.58(↑0.96) & 56.54(↑0.05) & 7.86(↑6.46) & 37.11(↑2.60) & 76.42(↑0.70) & 46.41(↑2.22) & 67.49(↑1.40) & 4.72(↑2.19) \\ \hline
 & \textbf{RG-1 + S-I} & 28.74(↑5.16) & 73.68(↑3.90) & 39.31(↑7.11) & 66.81(↑5.46) & 2.51(↑0.82) & 45.83(↑5.64) & 81.26(↑2.36) & 56.92(↑6.32) & 75.73(↑4.50) & 2.42(↑0.75) \\
 & \textbf{RG-1 + S-LS} & 26.83(↑6.55) & 71.07(↑4.76) & 37.64(↑9.02) & 63.80(↑7.31) & 2.16(↑0.76) & 40.77(↑6.26) & 78.36(↑2.64) & 50.84(↑6.65) & 71.07(↑4.98) & 1.93(↓0.60) \\
 & \textbf{RG-1 + S-D} & 19.67(↑6.58) & 66.66(↑4.45) & 28.78(↑8.05) & 58.65(↑6.52) & 6.62(↑2.29) & 38.94(↑8.05) & 77.38(↑3.63) & 48.82(↑8.92) & 70.21(↑6.84) & 9.20(↓0.41) \\
 & \textbf{RG-1 + S-P} & 18.14(↑10.41) & 67.18(↑6.86) & 26.47(↑12.77) & 56.38(↑10.60) & 9.71(↑3.47) & 36.67(↑10.55) & 76.81(↑4.35) & 46.41(↑11.52) & 66.76(↑8.56) & 6.43(↑2.20) \\
 & \textbf{RG-1 + S-I-D} & 27.60(↑3.62) & 71.29(↑3.09) & 36.54(↑5.12) & 64.93(↑4.53) & 6.73(↑0.86) & 47.61(↑4.72) & 81.43(↑2.19) & 58.60(↑5.35) & {\ul \textbf{77.14(↑3.58)}} & 9.30(↓0.40) \\
 & \textbf{RG-1 + S-I-P} & {\ul \textbf{30.26(↑5.17)}} & {\ul \textbf{73.81(↑3.71)}} & {\ul \textbf{40.30(↑7.36)}} & {\ul \textbf{67.47(↑5.55)}} & 11.35(↑2.32) & {\ul \textbf{48.24(↑6.51)}} & {\ul \textbf{81.80(↑2.91)}} & {\ul \textbf{58.89(↑7.13)}} & 76.25(↑5.05) & 8.38(↓2.95) \\
 & \textbf{RG-1 + S-LS-D} & 25.80(↑4.99) & 68.55(↑3.93) & 34.95(↑6.42) & 61.36(↑5.79) & 9.54(↑3.84) & 41.16(↑6.12) & 78.20(↑2.74) & 51.18(↑6.36) & 71.29(↑4.91) & 9.70(↑0.10) \\
\multirow{-8}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Retrieval\\  + \\ Static\\ Analysis\end{tabular}}} & \textbf{RG-1 + S-LS-P} & 27.94(↑5.60) & 70.77(↑4.24) & 37.62(↑8.04) & 63.16(↑6.62) & 9.23(↑1.37) & 44.05(↑6.94) & 78.92(↑2.50) & 53.64(↑7.23) & 72.11(↑4.62) & 6.94(↑2.22) \\ \hline

\end{tabular}
\end{adjustbox}
\end{table*}
